Adaptive Combinatorial Allocation

We consider settings where an allocation has to be chosen repeatedly, returns are unknown but can be learned, and decisions are subject to constraints. Our model covers two-sided and one-sided matching, even with complex constraints. We propose an approach based on Thompson sampling. Our main result is a prior-independent finite-sample bound on the expected regret for this algorithm. Although the number of allocations grows exponentially in the number of participants, the bound does not depend on this number. We illustrate the performance of our algorithm using data on refugee resettlement in the United States.

==> Sections/conclusion.tex <==
% !TEX root = ../adaptive_matching.tex
\section{Conclusion}
\label{sec:conclusion}


==> Sections/extensions.tex <==
% !TEX root = ../adaptive_matching.tex
\section{Extensions}
\label{sec:extions}


% 
% \subsection{Inference on counterfactual assignment mechanisms}
% 
% \MaxCom{Bayesian or unbiased? Or both?}
% 
% 
% \subsection{Theoretical characterization}
% 
%  compare performance to other (sub-optimal) procedures
% 
%  maybe focus on discrete covariates?
% 
% do reinforcement as an extension after that doesn't require a result? (and don't do review before)
% 
% \section{Calibrated simulations}
% 
% 
% Plan:
% \begin{itemize}
%   \item Estimate $\theta$ function from the available data.
%   \item Then simulate data based on this estimated function.
%   \item Do so for different possible matching mechanisms (randomized, our proposed algorithm, something like what you are doing thus far?)
% \end{itemize}

==> Sections/review.tex <==

\subsection{Matching and integer programming}
Here we think of the within-period matching problem, so we can drop the $t$ subscript. There are $k=1,\ldots,K$ refugee ``types''. All localities are assumed to be of different types (localities of the same type can be ``bundled'' together by adding their capacities).

There are $m^k$ refugees of type $k$, $m= \sum_k m^k$, and $n$ localities. We assume that in general $m\geq n$.

We want to identify the number of unique matchings to understand how big our action space is.
\subsubsection{One-to-one matching}

Recall that $m\geq n$. There are, therefore, \[ \frac{m!}{(m-n)!}\] one-to-one matchings. To see this, fix the order of the localities and permute the refugees, noting by for any of the $m!$ permutations of refugees, there are $(m-n)!$ permutation of the bottom refugees that result in the same matching.

Special case: when $m = n$, there are $n!=m!$ matchings.

\subsubsection{Unconstrainted many-to-one matching}

There are \[\binom{n+m^k-1}{n-1}=\binom{n+m^k-1}{m^k}\] ways to match $m^k$ indistinguishable refugees of type $k$ to $n$ localities.

There are, therefore,  \[\prod_k \binom{n+m^k-1}{n-1}=\prod_k \binom{n+m^k-1}{m^k}\] different matchings when there are no capacity constraints on localities.

\subsubsection{Constrainted many-to-one matching}
This is much harder.

\subsection{Multi-armed bandits and Thompson sampling}

\cite{Thompson2018}.

In each period $t$, assign treatment $d$ with probability $p_t^d$ equal to the posterior probability, given past outcomes, that it is in fact the optimal treatment,
\small
\begin{equation}
p_t^d=%P(D_t = d| \bs m_{t-1}, \bs r_{t-1}) = 
P\left (d = \argmax_{d'}  \theta^{d'} | \bs m_{t-1}, \bs r_{t-1} \right ).
\end{equation}
\normalsize
This prescription can be implemented by sampling one draw $\hat \theta_t$ from the posterior given the available information at time $t$, and setting 
$D_t = \argmax_d \hat \theta_t^d.$


In many bandit problems, the goal is to minimize average in-sample regret $E(\tfrac{1}{T}\sum_{t=1}^T \Delta^{D_{t}})$. 
%where $\Delta^d= \max_{d'} \theta^{d'} - \theta^{d}$.
\cite{agrawal2012analysis} (Theorem 2) have shown that in-sample regret for Thompson sampling (in the binary outcome setting, with sequential arrival) satisfies the bound
\be
\lim_{T\rightarrow \infty} E\left [\frac{\sum_{t=1}^T \Delta^{D_{t}}}{\log T}\right ] \leq \left (\sum_{d\neq d^{(1)}} \frac{1}{(\Delta^d)^2} \right )^2.
\ee
As first shown by \cite{lai1985asymptotically}, no adaptive experimental design can do better than this $\log T$ rate; the proof of this lower bound is reviewed in Section 2.3 of \cite{RegretBandit2012}.



\subsection{Dynamic programming and reinforcement learning}

\begin{itemize}
  \item Objective: Discounted stream of rewards, $\sum_{t\geq 0} \gamma^t R_t$.
  \item Expected future discounted reward at time $t$, given the state $S_t=s$:\\
 Value function,
  $$V_t(s) = E\left [\sum_{t'\geq t} \gamma^{t'-t} R_{t'} | S_t=s \right ] .$$
  \item Expected future discounted reward at time $t$, given the state $S_t=s$ \textbf{and} action $A_t=a$:\\
 Action value function,
  $$Q_t(a,s) = E\left [ \sum_{t'\geq t} \gamma^{t'-t} R_{t'} | S_t=s, A_t=a \right ] .$$
\end{itemize}


{Bellman equation}

\begin{itemize}
  \item Consider a policy $\pi(a|s)$, giving the probability of choosing $a$ in state $s$.\\
  This gives us all transition probabilities, and we can write expected discounted returns recursively
  $$Q_\pi (a,s) =  (\mathscr B_\pi Q_\pi) (a,s) =
  \sum_{s',r}  p(s',r| s, a) \left (r +  \gamma \cdot  {\color{blue} \sum_{a'} \pi(a'|s')}  Q_\pi(a',s')    \right ) .  $$
  
  \item Suppose alternatively that future actions are chosen optimally.\\
  We can again write expected discounted returns recursively  
  $$Q_* (a,s) = (\mathscr B_* Q_*) (a,s) =
  \sum_{s',r}  p(s',r| s, a) \left (r +  \gamma \cdot  {\color{red}\max_{a'}} \; Q_*(a',s')    \right ) .  $$
\end{itemize}


{Sarsa}

\begin{itemize}
  \item {\color{blue} On policy} learning of action value functions.
  \item Recall Bellman equation
  $$Q_\pi (a,s) =  
  \sum_{s',r}  p(s',r| s, a) \left (r +  \gamma \cdot  {\color{blue} \sum_{a'} \pi(a'|s')}  Q_\pi(a',s')    \right ).   $$
  \item Sarsa estimates expectations by sample averages.
  \item After each observation $\langle s, a ,r, s', {\color{blue} a'} \rangle$, replace the estimated $Q_\pi(a,s)$ by
  $$Q_\pi (a,s) + \alpha  \cdot  
  \left ( r +  \gamma \cdot Q_\pi({\color{blue} a'},s')  - Q_\pi (a,s) \right ).   $$
  \item $\alpha$ is the step size / speed of learning / rate of forgetting.
\end{itemize}

{Sarsa as stochastic (semi-)gradient descent}

\begin{itemize}
  \item Think of $Q_\pi(a,s)$ as prediction for $Y= r + \gamma \cdot Q_\pi(a',s')$.
  \item Quadratic prediction error:
  $$\left (Y -  Q_\pi(a,s) \right )^2. $$
  \item Gradient for minimization of prediction error for current observation w.r.t. $Q_\pi(a,s)$:
  $$- \left ( Y  - Q_\pi (a,s) \right ).   $$
  \item Sarsa is thus a variant of stochastic gradient descent. 
  \item Variant: Data are generated by actions where $\pi$ is chosen as the optimal policy for the current estimate of $Q_\pi$.
  \item Reasonable method, but convergence guarantees are tricky.
\end{itemize}

{Q-learning}

\begin{itemize}
  \item Similar to Sarsa, but {\color{red} off policy}.
  \item Like Sarsa, estimate expectation over $p(s',r|s,a)$ by sample averages.
  \item Rather than the observed next action $a'$ consider the optimal action ${\color{red} \argmax_{a'} }\; Q_*(a',s')$.
   \item After each observation $\langle s, a ,r, s'\rangle$, replace the estimated $Q_*(a,s)$ by
  $$Q_* (a,s) + \alpha  \cdot  
  \left ( r +  \gamma \cdot {\color{red} \max_{a'} }\; Q_*(a',s')  - Q_* (a,s) \right ) .   $$
\end{itemize}

{Approximation}

\begin{itemize}
  \item So far, we have implicitly assumed that there is a small, finite number of states $s$ and actions $a$, so that we can store $Q(a,s)$ in tabular form.
  \item In practically interesting cases, this is not feasible.
  \item Instead assume parametric functional form for $Q(a,s; \theta)$.
  \item In particular: Deep neural nets!
  \item Assume differentiability with gradient $\nabla_\theta Q(a,s; \theta)$.
\end{itemize}


{Stochastic gradient descent}

\begin{itemize}
  \item Denote our prediction target for an observation $\langle s, a ,r, s', {a'} \rangle$ by
  $$Y= r + \gamma \cdot Q_\pi(a',s'; \theta).$$
  \item As before, for the on-policy case, we have the  quadratic prediction error
  $$\left (Y -  Q_\pi(a,s; \theta) \right )^2. $$
  \item Semi-gradient: Only take derivative for the $Q_\pi(a,s; \theta)$ part, but not for the prediction target $Y$:
  $$- \left (Y -  Q_\pi(a,s; \theta) \right ) \cdot \nabla_\theta Q(a,s; \theta). $$
  \item Stochastic gradient descent updating step: Replace $\theta$ by
  $$\theta + \alpha \cdot \left (Y -  Q_\pi(a,s; \theta) \right ) \cdot \nabla_\theta Q(a,s; \theta).$$
\end{itemize}



\subsection{Gaussian process priors}


We assume that the policy maker has a prior for $m(\cdot)$ which takes the form
\begin{equation}
m(\cdot) \sim GP(\mu(\cdot), C(\cdot,\cdot)),
\label{eq:GPprior}
\end{equation}
where $GP(\mu(\cdot), C(\cdot,\cdot)$ denotes the law of a Gaussian process which is such that $E[m(t)] = \mu(t)$ and $\Cov(m(t), m(t')) = C(t,t')$, and where both the mean function $\mu(\cdot)$ and the covariance kernel $C(\cdot,\cdot)$ are assumed to be differentiable.
We impose further that the policy maker's prior is such that the function $m(\cdot)$ is independent of the probability distribution $P_T$ of $T$.
Such priors are discussed in detail in \cite{williams2006gaussian}.




\paragraph{Posterior expectation of the average response function $m$}
Recall that we assume the availability of a random sample $Y_i, T_i$, $i=1,\ldots, n$, satisfying equation \eqref{eq:normality}. 
What is the posterior expectation $\widehat{m}(t)$ of $m(t)$ given such data?
Denote $\bs Y=(Y_1,\ldots, Y_n)$ and  $\bs T=(T_1,\ldots, T_n)$, and let
\begin{align}
\mu_i &= E[m(T_i)|\bs T] =  \mu(T_i),  \nonumber \\  
C_{i,j} &=  \Cov(m(T_i), m(T_j)|\bs T) =  C(T_i, T_j), \textrm{ and} \nonumber \\
C_i(t) &= \Cov(m(t), m(T_i) | \bs T)  =  C(t, T_i).  
\end{align}
Let furthermore $\bs \mu$, $\bs C(t)$, and $\bs C$ denote the vectors and matrix collecting these terms for $i,j=1,\ldots,n$.
Since our setting implies joint normality of $\bs Y$ and $m(t)$ conditional on $\bs T$, the posterior expectation of $m(t)$ takes the form of a posterior best linear predictor:
\begin{align}
\label{eq:BLP}
\widehat{m}(t)= E[m(t) | \bs Y, \bs T]
 &= E[m(t)|\bs T] + \Cov(m(t), \bs Y |\bs T) \cdot \Var(\bs Y | \bs T)^{-1} \cdot (\bs Y- E[\bs Y|\bs T]) \nonumber \\
&= \mu(t) + \bs C(t) \cdot \left [\bs C + \sigma^2 \bs I \right ]^{-1} \cdot (\bs Y-\bs \mu).
\end{align}  
Note that at the points $\bs T$ observed in the sample, the function $\widehat{m}$ is equal to the familiar posterior mean for a multivariate normal vector, $(\widehat{m}(T_1), \ldots, \widehat{m}(T_n))= \bs \mu + \bs C \cdot \left [\bs C + \sigma^2 \bs I \right ]^{-1} \cdot (\bs Y-\bs \mu)$. In between these observed points, the function $\widehat{m}$ provides an optimal interpolation based on the smoothness assumptions encapsulated in the covariance kernel $C$.
When $T$ is drawn from a continuous distribution, $\widehat{m}$ adapts to arbitrary functional forms for $m$ in large samples. When $T$ has finite support, prior smoothness assumptions continue to matter for interpolation even in the large sample limit. 


==> Sections/simulations.tex <==
% !TEX root = ../adaptive_matching.tex
\section{Simulation results}


The bound for expected average regret per capita in period $t$ implied by Theorem \ref{theo:bounding_thompson} is given by
$$\sqrt{\frac{1}{2}\tfrac{\options}{\batch} \cdot \left [ \log\left ( \tfrac{\options}{\batch} \right ) +1 \right ] } \cdot \left ( \sqrt{\period} - \sqrt{\period-1} \right ),$$
where for the examples below
$d = k^2$ and $m=n$.
Since for the examples, $n = k^2$, we get $d/ m = 1$. 

\begin{figure}

\def\k{3}
\def\n{9}

\caption{\k\ types, \n\ matches per period}  
\includegraphics[width=.7\textwidth]{../R/simulation_results/k\k_n\n_combined_plot.pdf}

\def\k{4}
\def\n{16}

\caption{\k\ types, \n\ matches per period}  
\includegraphics[width=.7\textwidth]{../R/simulation_results/k\k_n\n_combined_plot.pdf}
\end{figure}


\begin{figure}

\def\k{5}
\def\n{25}

\caption{\k\ types, \n\ matches per period}  
\includegraphics[width=.7\textwidth]{../R/simulation_results/k\k_n\n_combined_plot.pdf}

\def\k{6}
\def\n{36}

\caption{\k\ types, \n\ matches per period}  
\includegraphics[width=.7\textwidth]{../R/simulation_results/k\k_n\n_combined_plot.pdf}
\end{figure}


\begin{figure}

\def\k{7}
\def\n{49}

\caption{\k\ types, \n\ matches per period}  
\includegraphics[width=.7\textwidth]{../R/simulation_results/k\k_n\n_combined_plot.pdf}

\def\k{8}
\def\n{64}

\caption{\k\ types, \n\ matches per period}  
\includegraphics[width=.7\textwidth]{../R/simulation_results/k\k_n\n_combined_plot.pdf}
\end{figure}

